VisRAG: Vision-based Retrieval-augmented Generation on Multi-modality Documents

Retrieval-augmented generation (RAG) is an effective technique that enables large language models (LLMs) to utilize external knowledge sources for generation. However, current RAG systems are solely based on text, rendering it impossible to utilize vision information like layout and images that play crucial roles in real-world multi-modality documents. In this paper, we introduce VisRAG, which tackles this issue by establishing a vision-language model (VLM)-based RAG pipeline. In this pipeline, instead of first parsing the document to obtain text, the document is directly embedded using a VLM as an image and then retrieved to enhance the generation of a VLM. Compared to traditional text-based RAG, VisRAG maximizes the retention and utilization of the data information in the original documents, eliminating the information loss introduced during the parsing process. We collect both open-source and synthetic data to train the retriever in VisRAG and explore a variety of generation methods. Experiments demonstrate that VisRAG outperforms traditional RAG in both the retrieval and generation stages, achieving a 20--40% end-to-end performance gain over traditional text-based RAG pipeline. Further analysis reveals that VisRAG is efficient in utilizing training data and demonstrates strong generalization capability, positioning it as a promising solution for RAG on multi-modality documents. Our code and data are available at https://github.com/openbmb/visrag.

==> Tables/image-retrieval.tex <==

\begin{table}
    \centering
    \caption{Result on MS COCO.}
    \label{tab:image-retrieval}
    \begin{tabular}{ll}
    \toprule
         \textbf{Model}& \textbf{MS COCO Recall@5}\\
    \midrule
         SigLIP (off-the-shelf)& 60.34\\
         \ours{}-Ret& 66.21\\
    \bottomrule
    \end{tabular}
\end{table}

==> Tables/overall-old.tex <==
\begin{table*}
\centering
\small
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{l|ll|ll|ll|l}
\hline
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{c|}{\textbf{Text Models}} & \multicolumn{2}{c|}{\textbf{Vision Models}} & \multicolumn{2}{c|}{\textbf{Multi-modal Models}} & \textbf{? Models}\\
\cline{2-8}
& BM25 & bge-large & CLIP & SigLIP & UniVL-DR & MARVEL & \ours{} \\
\hline
DocVQA (single page) & & & & & & & \\
DocVQA (multi page) & & & & & & & \\
InfographicQA & & & & & & & \\
ArxivQA & & & & & & & \\
ArxivCap & & & & & & & \\
Visually-intensive PDFs & & & & & & & \\
K12 Textbooks (Visually-intensive) & & & & & & & \\
K12 Textbooks (Text-centric) & & & & & & & \\
DocBank (Visually-intensive) & & & & & & & \\
DocBank (Text-centric) & & & & & & & \\
ICML Poster & & & & & & & \\
ICML Paper & & & & & & & \\
NeurIPS Paper & & & & & & & \\
\hline
\end{tabular}}
\caption{
Overall results. (This table compares \ours{} with out-of-the-box zero-shot models.)
% The best results in the two-stage ranking group are marked \textbf{Bold}.
% \texit{Stat. sig. difference w/ paired t-test (p<0.05) c=coCondenser, b=BERT Re-ranker, m=monoT5}
% \cx{besides \# paras can you also add in the O() complexity (of LM inference calls) w.r.t. number of docs, to show that three-stage rankers are really costly.}
}
\label{tab:overall}
\end{table*}

==> Tables/supervised-old.tex <==
\begin{table*}
\centering
\small
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{l|l||ll|ll|l}
\hline
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{1}{c||}{\textbf{Text Models}} & \multicolumn{2}{c|}{\textbf{Vision Models}} & \multicolumn{2}{c|}{\textbf{Multi-modal Models}} & \textbf{? Models}\\
\cline{2-7}
& MiniCPM & CLIP & SigLIP & UniVL-DR & MARVEL & \ours{} \\
\hline
DocVQA (single page) & & & & & & \\
DocVQA (multi page) & & & & & &  \\
InfographicQA & & & & & & \\
ArxivQA & & & & & & \\
ArxivCap & & & & & & \\
Visually-intensive PDFs & & & & & & \\
K12 Textbooks (Visually-intensive) & & & & & & \\
K12 Textbooks (Text-centric) & & & & & & \\
DocBank (Visually-intensive) & & & & & & \\
DocBank (Text-centric) & & & & & & \\
ICML Poster & & & & & & \\
ICML Paper & & & & & & \\
NeurIPS Paper & & & & & & \\
\hline
\end{tabular}}
\caption{
Supervised results. (This table compares \ours with baseline models fine-tuned on the train set.)
}
\label{tab:supervised}
\end{table*}
